A Generative Deep Learning Approach to Stochastic Downscaling of Precipitation Forecasts

Despite continuous improvements, precipitation forecasts are still not as accurate and reliable as those of other meteorological variables. A major contributing factor to this is that several key processes affecting precipitation distribution and intensity occur below the resolved scale of global weather models. Generative adversarial networks (GANs) have been demonstrated by the computer vision community to be successful at super-resolution problems, i.e., learning to add fine-scale structure to coarse images. Leinonen et al. (2020) previously applied a GAN to produce ensembles of reconstructed high-resolution atmospheric fields, given coarsened input data. In this paper, we demonstrate this approach can be extended to the more challenging problem of increasing the accuracy and resolution of comparatively low-resolution input from a weather forecasting model, using high-resolution radar measurements as a "ground truth". The neural network must learn to add resolution and structure whilst accounting for non-negligible forecast error. We show that GANs and VAE-GANs can match the statistical properties of state-of-the-art pointwise post-processing methods whilst creating high-resolution, spatially coherent precipitation maps. Our model compares favourably to the best existing downscaling methods in both pixel-wise and pooled CRPS scores, power spectrum information and rank histograms (used to assess calibration). We test our models and show that they perform in a range of scenarios, including heavy rainfall.

==> extracted.tex <==
% \author{ 
%   \large Lucy Harris \\[-3pt]
%   \normalsize University of Oxford  \\[-3pt]
%     \normalsize	lucy.harris2@physics.ox.ac.uk \\[-3pt]
% \and
%   \large Andrew T. T. McRae \\[-3pt]
%   \normalsize University of Oxford  \\[-3pt]
%     \normalsize	andrew.mcrae@physics.ox.ac.uk \\[-3pt]
% \and
%   \large Matthew Chantry \\[-3pt]
%   \normalsize European Centre for Medium-Range Weather Forecasts  \\[-3pt]
%     \normalsize	Matthew.Chantry@ecmwf.int \\[-3pt]
% \and
%   \large Peter D. Dueben \\[-3pt]
%   \normalsize European Centre for Medium-Range Weather Forecasts  \\[-3pt]
%     \normalsize	Peter.Dueben@ecmwf.int \\[-3pt]
% \and
%   \large Tim N. Palmer \\[-3pt]
%   \normalsize University of Oxford  \\[-3pt]
%     \normalsize	tim.palmer@physics.ox.ac.uk \\[-3pt]
% }

 The two networks are trained simultaneously against each other (``adversarially”) and so the discriminator serves to improve the generative network, which is ultimately responsible for producing high-quality samples. This ``minimax" game means GAN training is notoriously challenging, and has resulted in a sizeable effort by many researchers to find manageable training methods.
 
 In super-resolution applications, GANs create realistic reconstructed high-resolution images.
  
 A GAN generator typically has a noise input, which allows the network to produce a distribution of sample images, or an ensemble, as the noise input is varied. A conditional GAN, or cGAN, has a further input, or condition, to both the generator and the discriminator~\cite{mirza2014conditional}. In the networks discussed in this paper, this condition is a lower resolution set of atmospheric fields. The networks are also given high-resolution orography data and a land-sea mask, since these are expected to affect local precipitation due to physical principles \cite{Holden2011}. The generator network is therefore guided to produce a range of plausible high-resolution predicted rainfall images, based on a given lower-resolution forecast. The ability of GANs to produce an ensemble of outputs is significant in this problem since both precipitation forecasting and super-resolution are under-constrained problems, with no unique solution. An ensemble of outputs provides an assessment of the certainty of the output, which is hugely important in forecasting applications.

A variational auto-encoder (VAE) is another type of deep generative network, and we were interested in how a VAE approach performs on this problem compared to GANs. A VAE consists of two parts: an encoder and a decoder. The input is fed to the encoder, which encodes a lower-dimensional representation in terms of random variables, often parameterised by the means and variances of normal distributions. These random variables are then sampled, using an external noise input, and the resulting vector of `latent variables' is passed into the decoder. The decoder then generates a high-resolution image from the latent variable input. An ensemble of images can be generated by repeatedly sampling the random variables, as with the GAN generator. The VAE casts the encoder and decoder as neural networks and attempts to learn the best encoding-decoding scheme using an iterative optimisation process, using a defined loss function. The selection of a useful loss function is therefore key to producing good results using a VAE, but we found this was a difficult task. Conventional loss functions such as mean squared error led to subdued, `blurry' forecasts, and even far more esoteric choices gave almost no improvement. We therefore developed a hybrid VAE-GAN model which, within the GAN framework, simultaneously trained a VAE generator alongside a discriminator. This produced much better results.


 example 5 is from 06:00-07:00 UTC of the 17\textsuperscript{th} April 2019, example 6 s from hour 18:00-19:00 UTC of the 16\textsuperscript{th} January 2019 and example 7 is from hour 10:00-11:00 UTC of the 25\textsuperscript{th} May 2019.


The standard training objective for a GAN is a \emph{minimax} game: 
\begin{equation}
    \mathcal{L} = \mathds{E}_x [\log(D(x))] + \mathds{E}_z [\log(1-D(G(z)))]
\end{equation}

The generator, $G$ tries to maximise this loss function, whilst the discriminator, $D$ tries to minimise it. The real data input is represented by $x$, and the noise input is represented by $z$. The term $D(x)$ therefore represents the discriminator's estimate of the probability that the real data instance $x$ is real. $\mathds{E}_x$ is then the expected value over all real data instances. Similarly, $G(z)$ represents the output of the generator when given an input of random noise, $z$. $D(G(z))$ is then the discriminator's estimate of the probability that the generated, fake instance is real, so that $\mathds{E}_z$ is then the expected value over all random inputs to the generator. This derives from the binary cross-entropy between the real and generated distributions.

In a Wasserstein GAN \citet{Gulrajani2017}, however, the loss function takes the form:
\begin{equation}
    \mathcal{L} = \mathds{E}_x [D(x)] - \mathds{E}_z [D(G(z))]
\end{equation}
It is based on the Wasserstein metric, or earth-mover distance:
\begin{equation}
\label{eq:wasserstein}
    \mathcal{W}(\mathds{P}_r, \mathds{P}_g) = \sup_{\norm{f}_L \leq 1} \mathds{E}_{x ~ \mathds{P}_r} [f(x)] - \mathds{E}_{x ~ \mathds{P}_g} [f(x)] 
\end{equation}

where $\mathds{P}_r$ is the real data distribution, $\mathds{P}_g$ is the generated data distribution, and $f$ is a K-Lipschitz function so that the discriminator D is constrained to be within the $\mathcal{D}$, the set of 1-Lipschitz functions: $D \in \mathcal{D}$. The discriminator solves the problem of finding the function $f$ that solves the maximisation problem in equation~\ref{eq:wasserstein}. The loss functions themselves are then simple: the discriminator has a loss function:

\begin{equation}
    \mathcal{L}_D = D(x) - D(G(z))
\end{equation}

The discriminator tries to maximise this function, i.e. it tries to maximise the difference between its output on real instances and its output on fake instances.

The generator has loss function:
\begin{equation}
    \mathcal{L}_G = D(G(z))
\end{equation}

The generator tries to maximise this function, i.e. it tries to maximise the output of the discriminator for the generated fake instances.
Wasserstein GANs are less vulnerable to getting stuck than minimax-based GANs, and avoid problems with vanishing gradients \citep{Arjovsky2017}. The earth-mover distance also has the advantage of being a true metric: a measure of distance in a space of probability distributions. The fact that the earth-mover distance is continuous and differentiable means that
we can train the discriminator to optimality \citep{Arjovsky2017}. The Wasserstein loss implies that the discriminator will aim to produce an output that is as large as possible for a generated, fake input, and as small as possible for a real input.


However, the theoretical justification for the Wasserstein GAN (or WGAN) requires that the weights throughout the GAN be clipped so that they remain within a constrained range. Implementing a k-Lipschitz constraint via  weight clipping can lead to undesirable behaviour and optimisation difficulties \citep{Gulrajani2017}. After \citet{Gulrajani2017} we enforce the Lipschitz constraint using a gradient penalty, since a differentiable function $f$ is 1-Lipschitz if and only if it has gradients with norm at most 1 everywhere. This gives us the loss function for WGAN-GP:

\begin{equation}
    \mathcal{L} = \underbrace{\mathds{E}_x [D(x)] - \mathds{E}_z [D(G(z))]}_{\textrm{original discriminator loss}} + \underbrace{\gamma \mathds{E}_{\hat{x}} [(\norm{\nabla_{\hat{x}}D(\hat{x})}_2-1)^2]}_{\textrm{gradient penalty}}
\end{equation}

where the gradient penalty coefficient $\gamma$ is introduced - $\hat{x}$ is a random sample from the probability distribution $\mathds{P}_{\hat{x}}$, which is implicitly defined by sampling uniformly along straight lines between a pair of points sampled from the real data distribution $\mathds{P}_r$ and the generated distribution $\mathds{P}_g$, since the optimal discriminator contains straight lines with gradient norm 1 connecting coupled points from $\mathds{P}_r$ and $\mathds{P}_g$ \citep{Gulrajani2017}. 

A \emph{conditional} GAN has an additional input condition to both the generator and the discriminator \citep{mirza2014conditional}. Instead of modelling the joint probability $P(x,y)$, conditional GANs model the \emph{conditional} probability  $P(x|y)$. The loss function for a vanilla GAN then becomes:

\begin{equation}
    \mathcal{L} = \mathds{E}_x [\log(D(x|y))] - \mathds{E}_z [\log(1-D(G(z|y)))]
\end{equation}

The loss functions for a conditional WGAN-GP, as employed in this paper, thus take the form:
\begin{equation}
  \mathcal{L}_{D} (x,y,z; \theta_D) = D(x|y) - D(G(z|y)|y) + \gamma (\norm{\nabla_{\hat{x}}D(\hat{x})}_2-1)^2
\end{equation}

\begin{equation}
  \mathcal{L}_{G} (y,z; \theta_G) = D( G \left( z|y \right)) 
\end{equation}
where $L_D$ and $L_G$ are the loss functions for the discriminator and the generator, respectively, and $\theta_D$ and and $\theta_G$ are the corresponding trainable weights, with a gradient penalty weight $\gamma = 10$, after \citet{Gulrajani2017}. The samples $\hat{x}$, used to calculate the gradient penalty term, are randomly weighted averages of the real and generated terms:
\begin{equation}
    \hat{x} = \epsilon x + (1 - \epsilon) G(z|y)
\end{equation}

where $\epsilon$ is randomly sampled from a uniform distribution between 0 and 1.
The generator and discriminator are trained adversarially, with the model alternating between training the discriminator for five iterations and the generator for one, after \citet{Kurach2019}. The Adam optimiser \citep{Kingma2014} is used for both the generator and the discriminator, with a learning rate of $10^{-5}$, with larger learning rates resulting in unstable training. 

\begin{equation}
  \frac{\lambda}{N} \norm{x_\textrm{true} - \frac{1}{P}\sum_{i=1}^P G \left( z_i|y \right) }_{2} ^{2},
\end{equation}
over different noise samples $z_1, \ldots, z_P$, where $N$ is the number of pixels, and $\lambda$ is a weighting parameter.

\begin{equation}
\gamma \left( \norm{\nabla_{\hat{x}}D \left( \hat{x} | y \right) }_2-1 \right) ^2,
\end{equation}
where the gradient penalty coefficient $\gamma$ is introduced, and $\hat{x}$ is a random sample from the probability distribution $\mathds{P}_{\hat{x}}$. Following \citeA{Gulrajani2017}, this is implicitly defined by sampling uniformly along straight lines between a pair of points sampled from the real data distribution $\mathds{P}_r$ and the generated distribution $\mathds{P}_g$, since the optimal discriminator contains straight lines with gradient norm 1 connecting coupled points from $\mathds{P}_r$ and $\mathds{P}_g$. 

The generator was trained with 400000 sequences, corresponding to 3.2 million individual images, and the discriminator with 2 million sequences (10 million images). This corresponded to roughly 12 hours for each application, on an NVIDIA V100 GPU.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The computer vision community often employs the multi-scale structural similarity index (MS-SSIM) to assess whether the generated images accurately reproduce the spatial structure of the true images. The MS-SSIM is defined in \citet{Wang2003MSSSIM} by combining the SSIM across different scales, taking the reference and distorted image signals as the input, the system iteratively applies a low-pass filter and downsamples the filtered image by a factor of 2. The original image is indexed as Scale 1, and the highest scale as Scale $M$. :
\begin{equation}
    \textrm{SSIM} (\mathbf{x}, \mathbf{y}) = [l_M (\mathbf{x}, \mathbf{y})]^{\alpha _M} \cdot \prod^{M}_{j=1} [c_j \cdot (\mathbf{x}, \mathbf{y})]^{\beta_j} [s_j \cdot (\mathbf{x}, \mathbf{y})]^{\gamma_j}
\end{equation}
where $l_M (\mathbf{x}, \mathbf{y})$ is the luminance calculated only at scale $M$, $c_j$ and $s_j$ are the contrast comparison and structure comparison calculated at the $j$-th scale, respectively, and the exponents $\alpha_M$  $\beta_j$ $\gamma_j$ are used to adjust for the relative importance of the different components. 

%%%%%%%%%%%%%%%%%%%%

\section{Deterministic model and predictions}
\label{sec:deterministic-predictions}

The architecture for the deterministic approach is shown in Figure~\ref{fig:deterministic}.

\begin{figure}
    \centering
    \includegraphics[width=6cm]{Figures/deterministic.jpg}
    \caption{Network architecture for the deterministic approach}
    \label{fig:deterministic}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=15cm]{Figures/predictions-deterministic.png}
    \caption{Deterministic model output prediction examples for different input conditions}
    \label{fig:deterministic-prediction}
\end{figure*}

We can train the generator network architecture as a standalone model using mean squared error (MSE) as a loss function. The architecture for this network is displayed in Figure~\ref{fig:deterministic}. This CNN-based deterministic approach can be employed as a benchmark for a straightforward comparison to the GAN.

Example predictions for the deterministic model for different input conditions are shown in Figure~\ref{fig:deterministic-prediction}. In the case of the deterministic model, the example prediction is exactly the same as the mean prediction since. In the cases displayed here, the deterministic model prediction is arguably worse than the IFS forecast used as the input.

\begin{figure*}
    \centering
    \includegraphics[width=15cm]{Figures/predictions-deterministic-superresolution.png}
    \caption{Deterministic model output prediction examples for different input conditions, for the pure downscaling problem.}
    \label{fig:deterministic-prediction-easy}
\end{figure*}

Figure~\ref{fig:deterministic-prediction-easy} shows the deterministic results for the pure downscaling problem. Even the simple deterministic model performs very well on this problem. This again highlights the difficulty of the bias-correction element in addition to downscaling the forecast.

%%%%%%%%%%%%%%%%%%%%

The fifth example (Figure~\ref{fig:GAN-prediction}.5) is from 06:00-07:00 UTC of the 17\textsuperscript{th} April 2019 and  shows very little rainfall, with only one notable patch of rain in the IFS forecast, in the far north of the UK.
The IFS forecast completely misses this patch of rainfall, only predicting a small amount of very light rainfall over the North Sea. The three example GAN predictions show a significant variation, corresponding to the uncertainty in the situation. Whilst all three predictions show rainfall over the North Sea that is over a much larger area than the NIMROD data, the GAN models do predict some rainfall over the very north of the country. However, in all three cases it is too far west and not widespread enough. This situation is the example the GAN model struggles with most.

The sixth example (Figure~\ref{fig:GAN-prediction}.6) is from hour 18:00-19:00 UTC of the 16\textsuperscript{th} January 2019 and  shows three separate patches of rainfall on the large scale: a broad patch stretching over the north of Scotland, from the Highlands to the North Sea, a patch of rain in the south-west over the Irish Sea, Brecon Beacons and the Pennines, and a smaller patch of rainfall in the south-east over Kent and the Channel. There is intense rainfall in the patch to the south-west, particularly over the western coast of Wales. There is further intense precipitation near Aberdeen. The IFS forecast correctly captures the broad-scale structure of these three areas. The band of light rainfall to the south-east is a close match to the NIMROD data. However, the areas of precipitation to the north and south-west are over-predicted in terms of area whilst being under-predicted in terms of intensity. This is particularly noticeable over the west coast of Wales where there are bands of intense rainfall in the NIMROD data that look very different to the IFS forecast. The GAN model predictions are similarly well-calibrated for both intensity and spread for the rainfall over the Channel. The rainfall in the south-west shows the same intensity and structure as the NIMROD data. The rainfall over Scotland shows a fair amount of variation between ensemble members, but each prediction on its own is an improvement on the IFS forecast, and most importantly, two of the three ensemble members capture the more intense precipitation near Aberdeen.

The final example (Figure~\ref{fig:GAN-prediction}.7) is from hour 10:00-11:00 UTC of the 25\textsuperscript{th} May 2019 and shows a single large patch of precipitation over north-western Scotland, with small areas of higher intensity rainfall over the Highlands. The IFS forecast shows the same general structure, although there is rain forecast over the south of the UK as well as Ireland that is not present at all in the NIMROD data. The IFS forecast also fails to capture the fine-scale structure and small areas of high intensity over the Highlands. The GAN model predictions somewhat omit the spurious rainfall over the south of the UK and Ireland, with the correct situation displayed in at least one ensemble member each time. The large patch of precipitation over the Highlands and much of Scotland is a close match for the NIMROD data, both in terms of overall structure but also the small areas of higher intensity precipitation, likely due to local orographic variation, that appear on all the GAN model realisations.


%%%%%%%%%% ARCHITECTURE

Our basic residual blocks pass their input through two $3 \times 3$ convolutional layers, with multiple filters, and then add the input to the result of this -- a shortcut connection \cite{He2015}. Consequently, an inactive residual block, in which the convolutional layers have no effect, will act as an identity map. This theoretically allows the network to use more parameters as training progresses, without harming the initial development of the model, since an inactive residual block will pass the input straight through. We modify these residual blocks slightly by not passing the input straight through, but instead applying a pointwise ($1 \times 1$) convolution. This increases the capacity of the network slightly, and provided a small but consistent improvement in model skill.

After the input layer, the tensors are processed through the following steps:

\begin{enumerate}
\item Encoding:
    \begin{enumerate}
        \item The high-resolution geographic `constant' fields are encoded into a much larger number of channels, using convolutional layers, while bringing the image dimensions down to match the low-resolution input dimensions.
        \item The low-resolution input condition, the encoded constant fields, and noise channels are concatenated together.
        \item The generator inputs are then processed through a series of three residual blocks, each with $f_g$ filters, where $f_g$ is the number of filters applied in the generator and is a parameter that can be varied.
    \end{enumerate}
\item Upsampling and decoding:
    \begin{enumerate}
        \item The encoded representation of the generator inputs is passed through a series of two alternating upsampling and residual layers. Each upsampling pass increases the spatial dimensions, using bilinear interpolation. The first pass increases the resolution by a factor of five, and the second by a factor of two, for an overall increase in resolution by a factor $K = 10$. The two residual blocks operate with $2 f_g$ and $f_g$ channels respectively.
    \end{enumerate}
\item High resolution concatenation and encoding:
    \begin{enumerate}
        \item The full-size, high-resolution constant fields are re-introduced, and are concatenated with the output of the previous step, the upsampled, highly-processed input representation. This ensures the network has ample opportunity to benefit from the full-resolution geographic data.
        \item The high-resolution representation is processed through a further three residual blocks.
    \end{enumerate}
\item Output:
The output of the last hidden layer is mapped using a final convolution to a high-resolution tensor with dimensions $(b \times h_h \times w_h \times 1)$. This corresponds to precipitation values, at least in a transformed variable. A softplus activation in the final layer is used so that the network cannot produce a negative output, but the normalised prediction is not constrained on the upper end. The softplus activation function is also smooth, unlike ReLU, which has a discontinuous gradient.
\end{enumerate}

The inputs to the discriminator are the low-resolution input conditioning fields, the high-resolution constant fields (land-sea mask and orography) and a high-resolution input, passed as a 4-D tensors with dimensions $(b \times h_l \times w_l \times N_i)$, $(b \times h_h \times w_h \times 2)$, and $(b \times h_l \times w_l \times 1)$ respectively. The task of the discriminator is to distinguish the high-resolution ground-truth images from those produced by the generator. To achieve this, the discriminator network splits the inputs into a low-resolution and a high-resolution pathway. After the input layer, the tensors are processed through the following steps:

\begin{enumerate}
\item Encoding:
    \begin{enumerate}
        \item The high-resolution constant fields are encoded into a larger number of channels using convolutions, bringing the image dimensions down to match the low-resolution conditioning input dimensions.
        \item The low-resolution input condition to the network, encoded constant fields, and noise channels are concatenated together.
        \item The low-resolution discriminator inputs are then processed through a series of two residual blocks, to encode the information into a deep representation, with dimensions $(b \times h_l \times w_l \times 2f_d)$, where $f_d$ is the number of filters in the discriminator, a parameter that can be varied.
        \item The high-resolution constant fields are separately concatenated to the high-resolution input image. 
        \item The high-resolution discriminator inputs are processed through a series of downsampling convolutional layers, bringing the spatial dimensions down to match those of the low-resolution inputs, so that the dimensions of this pathway are also $(b \times h_l \times w_l \times 2f_d)$.
    \end{enumerate}
\item Combination:
The high-resolution and low-resolution pathways are concatenated.
\item Further encoding:
The output of the previous step is then processed through two residual blocks to reach a deeper representation.
\item Global average pooling:
The average of the feature map is taken, resulting in a tensor with dimensions $(b \times f_d)$
\item Output:
The output of the last layer is mapped using dense layers to a single output score.
\end{enumerate}


As with the GAN model, the inputs to the models are the low-resolution conditioning fields, the high-resolution constant fields (land-sea mask and orography) and a noise input, passed as a 4-D tensors with dimensions $(b \times h_l \times w_l \times N_i)$, $(b \times h_h \times w_h \times 2)$, and $(b \times h_l \times w_l \times n)$ respectively. During training, the low-resolution input image again has dimensions $(20 \times 20)$ and the high-resolution target image has dimensions $(200 \times 200)$ for a downscaling factor $K = 10$. 
